Learning the Regularization in DCE-MR Image Reconstruction for Functional Imaging of Kidneys

Kidney DCE-MRI aims at both qualitative assessment of kidney anatomy and quantitative assessment of kidney function by estimating the tracer kinetic (TK) model parameters. Accurate estimation of TK model parameters requires an accurate measurement of the arterial input function (AIF) with high temporal resolution. Accelerated imaging is used to achieve high temporal resolution, which yields under-sampling artifacts in the reconstructed images. Compressed sensing (CS) methods offer a variety of reconstruction options. Most commonly, sparsity of temporal differences is encouraged for regularization to reduce artifacts. Increasing regularization in CS methods removes the ambient artifacts but also over-smooths the signal temporally which reduces the parameter estimation accuracy. In this work, we propose a single image trained deep neural network to reduce MRI under-sampling artifacts without reducing the accuracy of functional imaging markers. Instead of regularizing with a penalty term in optimization, we promote regularization by generating images from a lower dimensional representation. In this manuscript we motivate and explain the lower dimensional input design. We compare our approach to CS reconstructions with multiple regularization weights. Proposed approach results in kidney biomarkers that are highly correlated with the ground truth markers estimated using the CS reconstruction which was optimized for functional analysis. At the same time, the proposed approach reduces the artifacts in the reconstructed images.

==> tex/method.tex <==

This manuscript proposes an image reconstruction method based on the extension of deep image prior technique to dynamic contrast enhanced MR image reconstruction. The method generates a regularized dynamic sequence of volumes given a corrupted dynamic series of images from undersampled the k-space measurement.  This section first explains the data acquisition details and the structure of the input and output data. The section then continues with the explanation of the proposed DIP based DCE-MRI reconstruction approach. 

\subsection{Data}
\label{subsec:Method-Data}
We acquired DCE-MR images using a work in progress (WIP) sequence from 10 patients (8 female, 2 male, age=6.5$\pm$4.9 years) who underwent a contrast-enhanced MRI exam \cite{coll2021modeling,coll2020bulk} for their clinical evaluation. All data were acquired following an approved IRB protocol and after obtaining consent.  We used a “stack-of-stars” 3D FLASH prototype sequence with a multi-channel body-matrix coil (3T Siemens Skyra/Prisma/Trio, TR/TE/FA=3.56/1.39~ms/12$^{\circ}$, 32 coronal slices, voxel size=1.25x1.25x3~mm$^3$, 3978 radial spokes acquired in 6.24 minutes with golden angle radial ordering), average temporal resolution was 3.2~s/volume.After 20 seconds of imaging, a contrast agent (gadobutrol, 0.75~ml/kg, Bayer HealthCare, Whippany, NJ) was power-injected intravenously. The kspace measurements were collected ans used in the reconstruction. Due to the high temporal resolution acquisition, original images were corrupted by noise and artifacts, which are regularized by the proposed method.


\subsection{Approach}
\label{subsec:Method-Approach}
Deep Image Prior (DIP) is a convolutional neural network (CNN) used to recover an  improved quality image given a corrupted image without using any prior training data other than the image itself. DIP technique uses a lower dimensional input which is passed through the convolutional neural network to generate a reconstruction candidate. Through the iterations of the learning process, generated image eventually captures an artifact or noise free reconstruction and ultimately the network overfits to the noisy observation. In DIP technique, the CNN structure is used as prior information to regularize the output and to remove noise and artifacts. For MR image reconstruction, we start from a lower dimensional representation $z_t$, and at each iteration an image $x_t$ is reconstructed to match its respective kspace measurement $k_t$ using Eqn.~\eqref{eq:dip_perspective}.

In DCE-MRI, dynamic sequence of images are temporally correlated. We design a lower dimensional input sequence $z$ to represent the temporal dynamics of the contrast enhanced image sequence. Given this lower dimensional input sequence, and a corrupted sequence of DCE-MRI images from undersampled kspace measurement through the forward model, our generator network parameters are optimized to reconstruct a regularized sequence of DCE-MR images with improved image quality, while at the same time preserving the temporal dynamics of the signal.
 
\noindent\textbf{Designing a lower dimensional representation:} Temporal signal in DCE-MRI can be separated into multiple phases such as no contrast phase, arterial phase, and the phases where different compartments and tissues enhance. To model this structure of temporal signal, we introduce a piece-wise linear $Z = \lbrace z_t| \forall t\in\lbrace1,\cdots,T \rbrace\rbrace$ design where each line segment represents the time correlation in a separate contrast phase.  To determine such structure, we use the i-NUFFT reconstructions of the dynamic sequence using Eqn.~ \eqref{eq:least_squares}: $X_{\text{ift}}=\lbrace {(FC)}^{-1}(k_t) | \forall t\in\lbrace1,2,\cdots,T \rbrace \rbrace$.

i-NUFFT reconstruction is computationally inexpensive and vectorized absolute images $|\text{vec}((FC)^{-1}(k_t))|$ form a reasonable foundation to capture the correlation between consecutive time frames. Let $\bar{X} = [|\text{vec}(x_t)|]_t\in \mathbb{R}^{n^2\times T}$ denote the concatenated absolute value of vectorized reconstructions. Our approach utilizes ordered principal components $w_s$s (because of principal component analysis (PCA)) and respective projections ${w_s}^T \bar{X}\in\mathbb{R}^T\ \forall s$ serve as different descriptors. Thresholding a descriptor defines a proximity of reconstructions, hence allows an empirically defined set of consecutive time samples e.g. $\lbrace t, t+1 ,\dots, t+c \rbrace \subseteq \lbrace 1,2,\cdots,T \rbrace$.  $Z$. Each component includes time indices that represent respective observations $k_t$s. A constant length line segment is generated for each component on which $z_t$s are placed in equidistant fashion. Determining $z_t$ is illustrated and summarized in Fig.\ref{fig:z_deisgn}.


\input{tex/experiments/performance_eval}

